Anchored, Not Graded: Vision-Language Models Fail at Slant-from-Texture Perception

Human perception of surface slant from texture exhibits systematic, graded biases that emerge reliably in psychophysical experiments. Prior work showed that unsupervised CNNs reproduce several human-like biases, while supervised CNNs do not. Do Vision-Language Models (VLMs) exhibit similar competences? Across multiple VLM families and model scales, zero-shot and in-context prompting both produce distinctive failures: slant is predicted at only a small set of anchors (e.g., 0\degree, $\pm$25\degree, $\pm$45\degree) with little dependence on stimulus field of view, optical slant, or surface curvature. Supervised fine-tuning partially remediates the failure, but residual anchoring persists. While success in high-level vision-language benchmarks might not require sensitivity to low-level geometric cues, we interpret anchoring as a failure at the representation-to-output language interface: not necessarily an absence of geometric encoding, but a failure to express it in a graded form.

==> tables/experimental_factors.tex <==

\begin{table*}[ht]
\caption{Experimental design factors for VLM slant estimation evaluation.}
\label{tab:experimental_factors}
\centering
\begin{tabular}{p{2.3cm}p{15cm}}
\toprule
\textbf{Experimental Factor} & \textbf{Description} \\
\midrule
Model & Vision-language models from different architectures and parameter scales (GPT-4V, Claude-3, LLaVA variants with 2B, 14B, 32B parameters) \\
Prompt Condition & Systematic variations in prompt content: presence/absence of visual cues, explicit mention of image attributes, and response format specifications \\
Visual Stimulus & Polka dot textured surfaces (see \cref{tab:datasets} for complete parameter specification) \\
Trial & Single presentation of the complete stimulus set to a given model under a specific prompt condition; multiple trials enable estimation of response reliability \\
\bottomrule
\end{tabular}
\end{table*}
